Wind power predictions from nowcasts to 4-hour forecasts: a learning approach with variable selection

We study short-term prediction of wind speed and wind power (every 10 minutes up to 4 hours ahead). Accurate forecasts for these quantities are crucial to mitigate the negative effects of wind farms' intermittent production on energy systems and markets. We use machine learning to combine outputs from numerical weather prediction models with local observations. The former provide valuable information on higher scales dynamics while the latter gives the model fresher and location-specific data. So as to make the results usable for practitioners, we focus on well-known methods which can handle a high volume of data. We study first variable selection using both a linear technique and a nonlinear one. Then we exploit these results to forecast wind speed and wind power still with an emphasis on linear models versus nonlinear ones. For the wind power prediction, we also compare the indirect approach (wind speed predictions passed through a power curve) and the indirect one (directly predict wind power).

==> sections/section4.tex <==
In this section, we compare several machine learning algorithms for predicting short term wind speed at the farms' location combining in situ variables and NWP variables using the variable selection methods presented in Section \ref{sec:varsel}.

%Many studies have been made on the subject of predicting local wind speed using machine learning techniques (see for instance Section 2 from \citet{TascikaraogluUzunoglu14} and references therein as well as Table 1 from \citet{AzimiAl16}). More recently, more complex and specialized approaches have been developped, such as \citep{RonayAl16, KhosraviAl18}, to focus on the most recent ones. The above is indeed far from exhaustive given the amount of such studies.
%% Most of those however generally do not make use of NWP forecasts and focus either only on very short or longer and less precise time horizons than we do. Moreover, the issue of variable selection is rarely investigated. Finally, kernel methods and particularily support vector machines (SVM) are especially popular in many studies, however the issue of their scalability is not investigated.
%\begin{itemize}
%\item \citep{RonayAl16}
%\begin{enumerate}
%\item Hourly (1 hour ahead prediction)
%\item Pure autoregressive
%\item 3 datasets but very small (2 months)
%\item Prediction intervals
%\item MLP + genetic and extreme ML + nearest neighbors
%\end{enumerate}
%
%\item \citep{KhosraviAl18}
%\begin{enumerate}
%\item 5min, 10min, 15min 30min
%\item Pure autoregressive
%\item 1 dataset, very small (a few days of data)
%\item Feedforward NN, SVR (linear), Fuzzy inference, Fuzzy inference + NN, blabla beaucoup de trucs chelous
%\end{enumerate}
%
%\item \citep{FengAl17}
%\begin{enumerate}
%\item 1 hour ahead
%\item 4 local variables
%\item 6 datasets of 1 year, 1min resolution
%\item Complex multimodel with feature selection
%\end{enumerate}
%
%\end{itemize}
%
%We propose here to adopt a global point of view, which may better fit the need of a practician wishing to use machine learning tools for predicting wind speed in the short term. First, we study many time horizons in an interval that can be of relevance for the energy market (10min-4h every 10min) \dimitri{Citation}. Second, for those time horizons, we focus on methods that are well known in the machine learning community for which highly efficient implementations are readily available and which scale very well with the number of datapoints (notably for kernel ridge regression, we investigate the scalability issue both for variable selection and for regression per se). 
%
%In that way, we aim a getting an overall view of what types of methods work well in which situations. Up to our knowledge, no such study has been performed before. Finally, we highlight that the significance of our results is increased by our averaging over several data splits as well as by the coherence of the results observed across six differents wind farms. 

\subsection{Non machine learning benchmarks and evaluation metrics}
\florence{what do you mean by non machine learning ? I understand but we may find another way to say it}
\riwal{Using persistence is an evident benchmark; the other relevant benchmark here is the NWP output, and this is rather original relative to many other studies of short-term wind speed forecasting; so I would suggest 'NWP benchmark and evaluation metrics', or 'Weather forecast benchmark and evaluation metrics'; it is implicit that persistence will be considered\dots}
First to evaluate the results, we consider the following metric. For a given wind farm, let $(y_i)_{i=1}^n$ denote the realizations of our target variable (the wind speed). We define the global mean as $\bar y:= \frac 1 n \sum_{i=1}^n y_i$.  Given a set of predicted values $(\widehat y_i)_{i \in  I}$ and a set of target values $(y_i)_{i \in I}$ where $I \subset \{1,...,n \}$, then we consider the Normalized Root Mean Squared Error (NRMSE) as it is defined in \citet{DupreAl20}:

$$ \text{NRMSE}: = \frac {\sqrt {\frac 1 {|I|} \sum_{i \in I} (\widehat y_i - y_i)^2}}{\bar y}. $$

\begin{figure}[H]
 	\centering
 	\includegraphics[width=0.6\linewidth]{./figs/pers_ecmwf_ws.pdf}
 	\caption{Persistence and ECMWF benchmarks for wind speed prediction.}
	\label{fig:non ml ws}
\end{figure}

\riwal{About figure \ref{fig:non ml ws}: the vertical axes should be the same; 
more importantly: does the performance of the ECMWF depend on time (more precisely, on how old the forecast is?)}

In particular, we want to measure the improvements that machine learning methods can bring over two simple benchmarks, namely persistence and ECMWF. The former predicts the last observed in situ wind speed, whereas the latter uses the wind speed at altitute 100m predicted by the NWP models using interpolation from ECMWF predictions. Persistence is expected to perform better in the short term whereas ECMWF will get better for longer time horizons, which is verified empirically on most wind farms as can be seen in Figure \ref{fig:non ml ws}. So as to quantify the improvements over persistence and ECMWF, let $S_{\text{pers}}$ be the NRMSE for the former on $I$ and let $S_{\text{ECMWF}}$ be that for the latter, we then define the following metric:

\begin{equation} \label{eq:delta nrmse}
\Delta \text{NRSME} := \frac {\min(S_{\text{pers}}, S_{\text{ECMWF}}) - \text{NRMSE} } {\min(S_{\text{pers}}, S_{\text{ECMWF}})}.
\end{equation}

\jordi{A forecast will be considered skill-full if  
DNRSME takes positive values}.

In itself, looking at the performances for the two non machine learning benchmarks in Figure \ref{fig:non ml ws} raises interesting questions. Indeed, the performance for persistence are quite similar from farm to farm. However, the quality of the ECMWF forecasts do vary tremendously. This could be explained in several ways. \dimitri{A controler/améliorer}. First, the geographical characteristics around of the different farms may play a role. Another possible explanation could be that the quality of the ECMWF forecasts vary from places to places. \riwal{I agree with the previous points, which may be expanded a bit; the following sentence can be removed: locations where data is assimilated can have special significance; otherwise, specific grid points are not more relevant than interpolated points in between, the scales of variation of the modelled fields are larger..} Finally we could also invoke the spatial resolution of ECMWF forecast, the resolution is 16 $\times $ 16 km, and thus we use linear interpolation to deduce forecasts at the farms' location; then depending on whether we are close or not to interpolation points, the quality of the obtained forecast can vary.
\jordi{ECMWF forecasting errors are lower for BM, BO and RE, which is consistent with the results in Figures \ref{fig:hsics} and \ref{fig:lasso}}, and it shows the better representation of NWP WS for these sites.

\subsection{Comparison of models for predicting wind speed}

We consider the following nonlinear methods: a kernel ridge regression with Nyström approximation (Nyström ridge), the well known optimized and improved boosted tree algorithm (XgBoost, \citet{ChenGuestrin16}) and a feed forward neural network (Feedforward NN). For those nonlinear methods, we use the 4 top features selected through BAHSIC \citep{SongAl12} on the training data as explained in Section \ref{subsec:hsic selection}. We also consider two linear benchmarks, the LASSO \citep{Tibshirani96} as well as an ordinary least square regression combined with forward stagewise variable selection (OLS f-stepwise) \citep{HastieAl01}. As in all our experiments, for the in-situ variables we consider 3h of past observations, and for the ECMWF ones we use prediction 1.5h before and 1.5h after the time horizon of interest. 

\begin{figure}[H]
 	\centering
 	\includegraphics[width=0.6\linewidth]{./figs/bench_ws.pdf}
 	\caption{Comparisons on WS forecasting}
	\label{fig:benchmarks ws}
\end{figure}

\riwal{Regarding figures \ref{fig:benchmarks ws} and \ref{fig:benchmarks pw}, 
I think it may be easier to read plots of NRMSE rather than $\Delta$ NRMSE. 
If we wish to keep a figure of $\Delta$ NRMSE, it could be a summary plot 
(one panel) showing six curves: the best $\Delta$ NRMSE (\dots) for each location }

For each data split, the key parameters of the different methods are chosen using the validation set (the regularization parameters, the Gaussian kernel parameter for the Nyström ridge, the number of variables for the forward stagewise linear regression, the architecture for the neural network ...). We do not give the full details here of all the parameters and the values we consider, however we provide such details in the supplementary material \dimitri{TODO}.

We display in Figure \ref{fig:benchmarks ws} the obtained results in terms of improvement over best non machine learning benchmarks---$\Delta \text{NRMSE}$ defined in Equation \eqref{eq:delta nrmse}. As a consequence, those results must be related to the scores of the persistence and ECMWF benchmarks displayed in Figure \ref{fig:non ml ws}. 

We observe that the methods that perform best on most farms are the Nyström ridge, the Lasso and the forward stagewise least square regression. The more complex nonlinear methods (XgBoost and Feedforward NN) are less efficient on this particular problem. Morever, for the neural network we do get a slight instability (results across time horizons are less smooth that for the other methods). We train different networks for each time horizon as it gives better results than training a single multi-output network, however the optimization variability for which neural networks are known, combined with highly correlated features, probably explains this unstability. On the other hand, linear models perform really well on the problem. In that regard, since the dynamics seems to be quite simple, our empirical results show that models for which we have low optimization error, such as the LASSO, the linear linear regression as well as the kernel ridge with Nyström approximation, are preferable. Nevertheless the much higher expressiveness of the latter model, may explain its slightly better performing on the majority of the farms. 

==> sections/section5.tex <==
\begin{figure}[H]
 	\centering
 	\includegraphics[width=0.6\linewidth]{./figs/power_curves.png}
 	\caption{Estimated power curves}
	\label{fig:power curves}
\end{figure}

We have two possibilities to predict energy production \citep{DupreAl20}. We can use the so-called indirect approach or the direct one. The first consists in training a model to predict wind speed first, and second to pass the result through a power curve. This power curve can be theoretical, however to better fit the characteristics of the different wind farms, we found it yielded better results to estimate it from the training data. The second method consists in directly training a model to predict energy production. However, since the power curves is a nonlinear transformation, we expect the linear methods will lack the necessary expressiveness to predict correctly energy production in a direct fashion, which is partially confirmed from the experiments in Section \ref{subsec:benchmarks pw}. 

\subsection{Indirect method}

Looking at the distribution in two dimension of energy production as a function of wind speed in Figure \ref{fig:power curves}, we observe numerous irregularities. The most notable ones being the presence of clamping of energy production which can be explained by several facts;  turbines can be clamped to reduce noise for instance at night, or they can be so to avoid material damage when wind speed is too high \dimitri{@Riwal, @Jordi, @Philippe je parle sous votre contrôle} \riwal{The last part can be removed; turbines are indeed stopped when winds are larger than the cut-off wind speed, but this is included in the power curve; the horizontal lines seen at BM, HC and RE look like curtailment; Christian Briard could confirm; do these values correspond to nightime? }. Since those are external events to which we do not have access directly in our database, we want to estimate the power curve without being too biased by those. A possible way to do so is to perform a nearest neighbor regression to predict energy production from wind speed. However, we can use the median instead of the mean in the prediction formula so as to estimate accurately the power curve in the absence of clamping. Examples of such estimated power curves are displayed in orange in Figure \ref{fig:power curves}. 

In the following section, we compare the methods that performed best for predicting wind speed in Section \ref{sec:ws forecasting} both in the indirect and the direct setting. 

\subsection{Non machine learning benchmarks and evaluation metric}
\begin{figure}[H]
 	\centering
 	\includegraphics[width=0.6\linewidth]{./figs/pers_ecmwf_pw.pdf}
 	\caption{Persistence and ECMWF benchmarks for energy production.}
	\label{fig:non ml pw}
\end{figure}

\jordi{I would suggest to merge figues 3 and 6 in one  figure}

When predicting energy production rather than wind speed, we want to measure the improvement over three non machine learning benchmark. We display the NRSME for those benchmarks in Figure \ref{fig:non ml pw}. As a comparison to the non machine learning benchmarks for predicting wind speed (see Figure \ref{fig:benchmarks ws}), the observations remain quite the same, except for the fact that depending on the wind farm, the direct persistence sometimes performs a tad better than the indirect one. The first two benchmarks correspond to the wind speed forecasts for persistence forecasts and ECMWF passed through the estimated power curves. For a given subset $I \subset \{1,...,n \}$, we denote by $S^{\text{ind}}_{\text{pers}}$ and $S^{\text{ind}}_{\text{ECMWF}}$ their respective NRMSEs on $I$. The third corresponds to direct persistence forecast for energy production, we denote its NRMSE on $I$ by $S^{\text{dir}}_{\text{pers}}$. Then to measure the improvement of a method over those three, we re-define $\Delta \text{NRMSE}$ as: 

$$ \Delta \text{NRSME} := \frac {\min(S^{\text{ind}}_{\text{pers}}, S^{\text{ind}}_{\text{ECMWF}}, S^{\text{dir}}_{\text{pers}}) - \text{NRMSE} } {\min(S^{\text{ind}}_{\text{pers}}, S^{\text{ind}}_{\text{ECMWF}}, S^{\text{dir}}_{\text{pers}})}.$$ 


\subsection{Comparison between direct and indirect methods} \label{subsec:benchmarks pw}

\begin{figure}[H]
 	\centering
 	\includegraphics[width=0.6\linewidth]{./figs/bench_pw.pdf}
 	\caption{Comparisons on PW forecasting}
	\label{fig:benchmarks pw}
\end{figure}

We now compare the methods that performed best to predict wind speed for predicting energy production (Nyström ridge, LASSO and OLS f-stepwise). For each method, we consider both direct and indirect method. We display the results in Figure \ref{fig:benchmarks pw} which must be related to the non machine learning benchmarks presented in Figure \ref{fig:non ml pw} to interpret correctly the $ \Delta \text{NRSME}$. 
We make the following observations: 
\begin{itemize}
\item The direct Nyström ridge is the method which performs the most consistently across farms. And on half of the farms (MP, RE, VE), it performs much better that the other methods for all time horizons.
\item  Except for very short lead times, on most farms, using linear methods to predict directly energy production does not work well. It can be explained by the nonlinearity of the power curves, even though one can assume that this is partially alleviated by the presence of past energy production in the input variables set.
\item For very short lead times, direct forecasting always seems to be preferable, notably on half of the farms (RE, VE, HC), all indirect forecasting methods perform much worse than persistence. 
\end{itemize}
